How to Data in Datathons

The rise of datathons, also known as data or data science hackathons, has provided a platform to collaborate, learn, and innovate in a short timeframe. Despite their significant potential benefits, organizations often struggle to effectively work with data due to a lack of clear guidelines and best practices for potential issues that might arise. Drawing on our own experiences and insights from organizing >80 datathon challenges with >60 partnership organizations since 2016, we provide guidelines and recommendations that serve as a resource for organizers to navigate the data-related complexities of datathons. We apply our proposed framework to 10 case studies.

==> content/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We have further clarified that data ethics is out of the scope of this paper.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Public available reports}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

\section{Appendix}

Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

\begin{enumerate}

\item Submission introducing new datasets must include the following in the supplementary materials:
\begin{enumerate}
  \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
  \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
  \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
  \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
\end{enumerate}

\item To ensure accessibility, the supplementary materials for datasets must include the following:
\begin{enumerate}
  \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
  \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
  \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
  \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
  \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
  \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
\end{enumerate}

\item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

\item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
\end{enumerate}

\end{document}


==> content/mysc.tex <==
% Here describe the process of finding out what Tier is the right one.
% Thinking about the outcomes you expect, there is a trade-off between usability (Tier 0) and security (Tier 4).
% [Here be Data Safe Haven Tier Classification]
% \begin{itemize}
%     \item Tier 0: These environments process publicly available data, ensuring its suitability for open handling. They do not involve personal, sensitive, or consequential information. Managed within a structured data analysis infrastructure, Tier 0 datasets instill stakeholder confidence, even when analyzed on personal devices. Including them in inventory and curatorial systems of a research data environment is essential. Audit trails play a crucial role in mitigating misclassification risks, providing transparency and accountability for data processing during misclassification periods.
%     \item Tier 1: These environments handle data intended for publication or that can be published without reputational damage, offering a competitive advantage to the research team. Privacy is maintained for strategic purposes rather than legal data protection requirements. The datasets and processing meet Tier 0 criteria. Tier 1 can involve anonymised or synthetic information derived from personal data, as long as high-quality anonymisation ensures it is no longer classified as personal data. However, pseudonymised data, which can be re-identified with a key or other datasets, is excluded. Commercial data with negligible or no impact on disclosure consequences can also be processed in Tier 1 with the agreement of all parties involved.
%     \item Tier 2: These environments handle non-personal data, including pseudonymised or synthetic information generated from personal data with strong confidence in the quality of pseudonymisation. The risks of re-identification and workaround breaches are considered during the classification process. Confidential information that is not sensitive in commercial or national security terms can also be processed in Tier 2, provided the potential consequences of disclosure are low. Tier 2 corresponds to the government's OFFICIAL classification.
%     \item Tier 3: These environments are dedicated to processing personal data, including pseudonymised or synthetic information with weak confidence in pseudonymisation. They also handle sensitive information in commercial, legal, political, or national security contexts, aligning with the government's 'OFFICIAL–SENSITIVE' classification. Tier 3 accounts for defending against attackers with limited capabilities, while excluding sophisticated threat actors. The distinction between Tier 2 and Tier 3 is critical for researcher productivity and organizational risk. In Tier 3, the risk of hostile actors attempting to breach the secure environment becomes significant.
%     \item Tier 4: Environments encompass the processing, combination, or generation of personal data with potential threats to the personal safety, health, or security of data subjects. This tier also involves handling sensitive datasets in commercial or national security contexts, which may attract the attention of sophisticated and well-resourced threat actors, including serious organized crime groups and state actors. In line with the UK government's classification, Tier 4 is designated as "SECRET." Notably, at Tier 4, the risk of hostile actors infiltrating the project team becomes significant.
% \end{itemize}

    %Primary risk is de-identification of the data. Satisfactory measures need to be taken to ensure annonymisation 
    % data which has been pseudonymised / synthetic information generated from personal data. The most significant risk is believing data is anonymised when re-identification might be possible.

        % Due to the level of personal or commercial risk associated, we do not support datathons in this tier.
    
    % Data which includes pseudonymised / synthetic information generated from personal data, where the classifier only has weak confidence in the quality of the pseudonymisation. Includes sensitive data (e.g. commercial, legal, political). Needs to account for potential attacks. 



% \subsection{Ethics}
% \carlos{I am unsure if this section should be kept. It needs to be mapped to the DSGs report. Also is not sitting in any prior work.}
% COMMENT: [[[Ethics on the data:Relate with the GDPR and AI ACT.]]]


% Projects considered for hackathon events must undergo ethical assessment prior to selection. It is essential to choose an assessment that adequately covers they key ethical dimensions during the intake stage evaluation of potential projects:
% \begin{itemize}
%     \item Data Ethics: Data ethics refers to the moral principles and guidelines governing the collection, storage, processing, and use of data. It involves considerations such as privacy, consent, transparency, fairness, and accountability. Data ethics seeks to ensure that data practices prioritize individuals' rights, avoid harm, and promote societal well-being. This stage has become even more important recently, on account of the recent developments in regulation surrounding data-based projects (GDPR) and AI in general (EU AI Act).
    
%     \item Project Definition Ethics: When ethically assessing a project proposal, it is essential to align it with the organization's codes of conduct, ethical guidelines, and values, ensuring consistency and integrity in decision-making. This involves evaluating if the proposal adheres to fairness, integrity, respect, social responsibility, and sustainability principles. Assessing the impacts on stakeholders is crucial, analyzing positive and negative consequences for employees, customers, communities, suppliers, and the environment, considering short and long-term effects and potential conflicts of interest. Broader moral and ethical considerations should be evaluated, such as human rights, social justice, environmental sustainability, and harm prevention. If the proposal conflicts with codes of conduct or ethical guidelines, the organization should communicate concerns and explore alternative projects aligned with its values. Ethical assessment enables responsible decisions upholding standards and benefiting society.
    
%     \item Project Execution Ethics: This area pertains to the manner in which a project is carried out, with a particular emphasis on addressing the human dimension involved. In certain instances, data-driven projects may utilize datasets that possess scientific relevance but have the potential to evoke emotional distress or offense among researchers. Such datasets might even pose a risk to the mental well-being of individuals involved. Notably, in hackathon events, this aspect assumes heightened significance compared to other project types, given that participants engage on a voluntary basis without any form of compensation or prior agreement explicitly expressing their consent or comfort with such data.
% \end{itemize}

###RELATED WORK

%In the next section, we discuss some existing work on data challenges and taxonomies in general contexts.

%We only mention a few works in this section. \citep{DBLP:conf/cscw/TrainerKCH16} conducted a case study of hackathons focused on scientific software development, highlighting the importance of face-to-face interactions and social ties.  \citep{DBLP:conf/chi/OlesenKH21} analyzed various hackathon formats and explored the causal relationships between input, process, and effects. \citep{falk_olesen_10_2020} identified key concerns in hackathon research, such as the impact of event structure on learning and research processes. \citep{DBLP:journals/pacmhci/NolteCH20} emphasized the importance of sustainability and continuity in hackathon projects. \citep{kollwitz_what_2019} developed a taxonomy of hackathon design decisions related to operational requirements and strategic goals.



% \carlos{Richard, I cute there. We can be more extensive in the appendix. Delete this comment once read.}
%\citep{DBLP:conf/cscw/TrainerKCH16} conducted a case study of three hackathons focused on scientific software development, analyzing team formation, collaboration, and social ties. The authors used 1:1 interviews with participants to collect data and analyzed the number of commits on GitHub during and after the event. Their study provides insights into the importance of face-to-face interactions and social ties in hackathon events.

%\citep{DBLP:conf/chi/OlesenKH21} analyzed 16 hackathons through research studies and provided a program theory analysis of hackathon formats, exploring causal relationships between input, process, and effects. They emphasized the democratizing potential of hackathons and cataloged various formats of hackathons. Their analysis focused on three main axes: participation, sustainable outcomes, and learning. They also considered the short- and long-term effects of hackathons, including immediate tangible and intangible products, short and midterm effects, and long-term impacts. They provide detailed tables analyzing each of the hackathons and their outcomes.

%This extended previous work \citep{falk_olesen_10_2020} which conducted a structured review of 381 hackathon-related publications created between 2000 and 2018. This work established the key concerns of hackathon research as falling into three areas: dealing with how the structure of such events impacts learning, research processes, and how they engage participants, notably through community organisation and increasing diversity. They also made the distinction between research conducted \textit{with} hackathons, which was primarily concerned with the tangible outcomes of the process, and research \textit{on} hackathons, which demonstrated more interest in how event design decisions influenced pedagogic experiences.

%\citep{DBLP:journals/pacmhci/NolteCH20} differentiated between short- and long-term continuation in hackathon projects and found that intensive short-term activity was associated with a lower likelihood of long-term project continuation. Their study highlights the importance of sustainability and continuity in hackathon projects.

%\citep{kollwitz_what_2019} conducted a systematic literature review including 189 publications in order to develop a comprehensive taxonomy of hackathon design decisions, categorised into those related to operational requirements, and those instrumental to strategic goals. The analysis related these factors to the range of expected outcomes and impacts desired by organisers, proposing this as the basis of a potential ontology of hackathon characteristics.

%While these studies do not focus specifically on datathons, they provide useful insights into related events and can inform our understanding of best practices and potential challenges for datathons.

% \citep{doi:10.1126/scitranslmed.aad9072} defined the term "datathon" as an application of cross-domain hackathon principles to objects of study amenable to data analytics, in their case study biomedical research datathons conducted in 2014 and 2015 using healthcare admissions data. The work primarily stresses the benefits of interdisciplinary study, claiming that this may help address poor study design, paucity of data, and improved analytical rigour through increased transparency.

% \citep{luo_mit_2021} reported the outcome of a virtual datathon conducted in 2020 across multiple institutions including the Massachusetts Institute of Technology and Beth Israel Deaconess Medical Center with the goal of generating insights about the early stages of the Covid-19 pandemic across multiple domains. Organisers designed a group of potential research questions, while allowing participants to define their own specific goals, utilising materials from among the publicly-available datasets on offer. Participants were selected for balanced gender representation, as well as team composition mix across data scientists, project managers, mentors, clinicians, and other subject matter experts.

% \citep{piza_assessing_2018} conducted a survey of participants in a 2017 healthcare-focused datathon hosted by a hospital in São Paulo, Brazil. The study demonstrated a significant association between participants' experience of positive teamworking behaviours and affective learning, pointing out effective leadership as the key factor. The paper asserts that a robust collaborative learning framework is correlated to affective values such as trust, adaptation, and member behaviour.


%The amount of data created each day across the globe doubles approximately every 40 months \citep{McAfee2012}. This clearly gives organizations the ability to work with huge datasets from different sources. However, although there is a heightened interest in the \textit{big data} phenomenon, does the assumption "the more, the better" hold?

%As mentioned by \citep{Sadiq2017}, apart from data quality concerns, there is a growing trend of aggregating vast amounts of data from diverse sources into loosely structured data management platforms referred to as \enquote{data lakes}. This practice can lead to a significant delay in extracting value from these datasets, primarily because of the limited scientific understanding available for efficiently evaluating the data and assessing its quality. Consequently, this often results in valuable information assets being underutilized.

% \citep{kuter_hosting_2021} reported the experience of running a hackathon with data of such sensitivity that participants were required to sign non-disclosure agreements, as well as purging all copies of the challenge dataset, which they cite as a drawback so significant that it led to the creation of bespoke datasets in all subsequent events. They also draw attention to the investment of time and resources in removing personally identifiable information (PII).



% Missing data is everywhere, yet rarely talked about explicitly. What makes Hackathons fun and efficient is quickly iterating through different ideas and analysis towards visible results rather than painfully spending days dealing with missing data. Yet, we now have solutions, mainly coming in two forms: multiple imputation (MI) and data augmentation (DA) \citep{nakagawa2015missing}. The question therefore is: How much and what type of missing data are still acceptable in Hackathon datasets? 

% Missing data theory provides three fundamental categories to think about the the mechanisms underpinning missing data \citep{rubin1976inference, little2002bayes}: missing completely at random (MCAR), missing at random (MAR) and missing not at random (MNAR) (but see \citep{gelman2006data} for a different classification). These missing data mechanisms describe the statistical relationship between the variables in a model and the probability of missing data.  Informally, data are MCAR when the probability of missing data in a variable isn't related to any other observed variable \citep{nakagawa2015missing}. MAR describes a mechanism where the probability of missing data in a variable is related to some other variable(s) in the data. While the "random" in MAR is somewhat confusing, one can think about it as 'conditionally missing at random', in that the missingness is random after controlling for other variables \citep{graham2009missing}. Lastly, missing data due to MNAR happens when the missing data is linked to the variable itself, even after taking into account the other observed data. For example, if in a study on coffee drinking, people who drink most coffee wouldn't answer the last questions because they were busy grabbing their next cup of coffee and got stuck in a chat with colleagues, the data would be Missing Not At Random (MNAR). Note that all these mechanisms also have formal definitions \citep{nakagawa2015missing}.

%**Something about diagnostics**
%Notably, of all three mechanisms the only one we can empirically test is MCAR \citep{baraldi2010introduction},

%**what to do **

%**summary on whats appropriate for hackathons**




% \textbf{Suitability}:

% It is based on our experience of running DSGs that we provide a framework to assess how \enquote{ready} a datathon is for participants to attend.

% \subsection{DSG Reports}
% % Don't know if this should be after the data assessment matrix, or in case studies directly.
% \carlos{This section needs improvement}
% We used the final reports, which are published on the Alan Turing Institute's website\footnote{\url{https://www.turing.ac.uk/collaborate-turing/data-study-groups}}, as a measure to analyse the effectiveness and success of a DSG. It is important to note that there is a bias in the publication of reports -- reports which pass a minimum quality criteria, as reviewed by the team, is published. Additionally, the initial reports from the early editions of the DSG may not be published, as the methodology was introduced in later iterations, so we focus on the later editions. 


% During the analysis of the reports, if multiple issues related to a specific data analysis dimension were identified, we considered the worst-case scenario.
% Not sure what this sentence adds


==> notes/clare_notes.tex <==
Lifecycle of hackathon;
- Before (preparation?)
- During (cannot effectively monitor any metrics / statistics during the event, besides qualitative feedback)
- After (not enough info / follow-up with companies not that feasible / could ask participants how DSG helped their career)

Perspective pieces;
https://www.nature.com/articles/s41467-020-15871-z 
https://ieeexplore.ieee.org/abstract/document/9592479?casa_token=TNPgsPs1v4sAAAAA:H3DzqRVIedYecfUb2xSVa_APB-zG0krPKJAQn-kHjwDz4d0M-MPqViAjp9OFxLGZzavGuLVy [Data Readiness Report]

Data frameworks;
https://link.springer.com/chapter/10.1007/978-3-030-43823-4_1
https://www.nature.com/articles/s41467-020-15871-z 

NLP frameworks;
https://arxiv.org/abs/2009.02043

Why datathons in the first place;
https://arxiv.org/pdf/1903.07539.pdf 



Areas that we could contribute?;
